MIRA: A Method of Federated MultI-Task Learning for LaRge LAnguage Models

In this paper, we introduce a method for fine-tuning Large Language Models (LLMs), inspired by Multi-Task learning in a federated manner. Our approach leverages the structure of each client's model and enables a learning scheme that considers other clients' tasks and data distribution. To mitigate the extensive computational and communication overhead often associated with LLMs, we utilize a parameter-efficient fine-tuning method, specifically Low-Rank Adaptation (LoRA), reducing the number of trainable parameters. Experimental results, with different datasets and models, demonstrate the proposed method's effectiveness compared to existing frameworks for federated fine-tuning of LLMs in terms of average and local performances. The proposed scheme outperforms existing baselines by achieving lower local loss for each client while maintaining comparable global performance.

==> related_work.tex <==
\section{Related work} \label{REW}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Federated Multi-Task Learning}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The problem of statistical heterogeneity often exists when training an FL system. In such cases, the performance of the global learned model might degrade unless a careful solution is introduced to deal with the heterogeneity of the data across clients~\cite{karimireddy2020scaffold}. One such solution is to cast the problem as a multi-task learning (MTL) problem, enabling different clients to learn different models, based on their tasks and data distribution while still leveraging the collective structure of other clients' tasks. Several approaches have been proposed that adapt MTL to model FL problems. For example, Smith \textit{et al.}~\cite{smith2017federated} were the first to propose the idea and introduced a method to solve the problem in the convex and strongly convex settings by solving a quadratic sub-problem locally at each client. In \cite{li2021ditto}, the authors aligned the local learned model and the global one using regularization improving, both, model personalization and fairness among clients. The existence of a hidden relationship between clients' models was assumed in \cite{9975151}, and the Laplacian matrix was leveraged to capture this relationship.
%In \cite{9975151}, the authors assumed the existence of a hidden relationship between clients' models and leveraged the Laplacian matrix to model such a relationship.
We build upon and extend this method, adapting the use of the Laplacian matrix to better suit the constraints of LLMs.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Parameter-Efficient Fine-tuning }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Traditional approaches for fine-tuning Deep Learning (DL) models are centered around two directions. The first is to take a pre-trained model, replacing only the classification head to suit the task in hand, making the parameters of this classification head trainable while keeping the rest of the architecture frozen. The second approach is to do full fine-tuning of the model, updating all parameters at hand. While the first approach is common among different problems, it is not always the case that such a method would allow the model to adapt to the new problem. In addition, for every task at hand, a new round of fine-tuning is needed. The other approach, while ideal for all cases, suffers from the large computational overhead that is associated with such pre-trained models. Parameter-efficient fine-tuning (PEFT) methods seek a middle ground by adding a small set of parameters to the pre-trained model and only training the newly added parameters. PEFT methods can be classified into three classes: Additive methods, which add a new set of layers or parameters to the pre-trained model and update those layers only. One example of the additive family is prompt tuning~\cite{lester2021power} where a prompt token is added to the pre-trained model, optimizing only the embedding of this token. The second family is the selective methods, where only a subset of the model's parameters are chosen to be updated. One such technique is BitFit~\cite{ben-zaken-etal-2022-bitfit}, which only updates the biases of the model while keeping the weights frozen. The third family of PEFT methods is the reparametrization-based methods. LoRA is an example of such a method, where the model parameters are decomposed into two smaller matrices that are optimized instead of the original weight matrix. We leverage LoRA as our PEFT method to reduce the computational overhead associated with LLMs.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Federated Fine-tuning of LLMs}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Multiple frameworks already exist to leverage FL for fine-tuning LLMs. For example, Zhang \textit{et al.} \cite{zhang2023fedpetuning}~proposed the usage of different Parameter-efficient fine-tuning methods like prompt tuning to make the fine-tuning process of LLMs communication efficient. The idea of prompt tuning is to add a set of virtual tokens, often called a soft prompt, to the original prompt, i.e., the hard prompt. It then tries to optimize the soft prompt to generate the desired output. In \cite{xu2023federated}, the authors made use of the fact that most FL settings operate with edge devices that are designed by nature for inference not training, leading to a zeroth-order utilization for the problem without the need for BP. LoRA~\cite{hu2021LoRA} was used in \cite{10447454} to reduce the number of parameters that need to be optimized. This significantly reduces the number of trainable parameters of the LLM and makes the computation more lightweight. A zeroth-order method that shares only two numbers, the scalar gradient and the seed used to generate the perturbation vector necessary to calculate the gradient, was proposed in \cite{malladi2023fine}. By limiting the number of seeds clients can use to $k$ seeds, each client can recover the latest global model by running at most $k$ local steps. Although this approach is communication-efficient, it introduces a computation overhead since each client needs to perform $k + R$ local steps to get the latest model and make a round of local updates for $R$ rounds. The main problem with the existing federated fine-tuning approaches for LLMs is the fact that they all learn a single global model based on model averaging, which might not be the optimal solution for highly heterogeneous settings. We address this problem by modeling the problem as an FMTL, instead, and learning a separate model per client.


